GANzilla: User-Driven Direction Discovery in Generative Adversarial Networks

Generative Adversarial Network (GAN) is widely adopted in numerous application areas, such as data preprocessing, image editing, and creativity support. However, GAN's 'black box' nature prevents non-expert users from controlling what data a model generates, spawning a plethora of prior work that focused on algorithm-driven approaches to extract editing directions to control GAN. Complementarily, we propose a GANzilla: a user-driven tool that empowers a user with the classic scatter/gather technique to iteratively discover directions to meet their editing goals. In a study with 12 participants, GANzilla users were able to discover directions that (i) edited images to match provided examples (closed-ended tasks) and that (ii) met a high-level goal, e.g., making the face happier, while showing diversity across individuals (open-ended tasks).

==> 08_conclusion.tex <==
\section{Conclusion}

==> 09_acknowledgements.tex <==



==> 99_recycle.tex <==
% recycled tex code



% \subsubsection{Closed-ended tasks}\hfill\\
% \textit{User Performance}

% As a baseline, we compare user-generated directions with the reference image (initial image). We expect the user-generated direction to result in a closer image to the target image than the reference image. We compare the average similarity between the reference direction (resulting in the reference image) and the target direction for each task. We then compare the average similarity between the user-generated directions and the target direction. We calculate the similarity as it is explained in Section~\ref{closed_ended_explanation}. 

% In both cases we use the VGG-Face model. The results are normalized between 0 and 1, where 1 refers to the identical directions. The goal of this comparison is to show that after applying the user-found directions, images get more similar to the target. Reference images have $0.388$, $0.252$ and $0.377$ similarity to the target images for closed task 1,2 and 3 respectively. Whereas, user-generated directions create images that have $0.446 \pm 0.123$, $0.422 \pm  0.112$ and $0.544 \pm 0.140$ similarity respectively. 


% Across all tasks, the mean and standard deviation of the similarity is $0.471 \pm 0.142$ for the closed-ended tasks which is better by $0.132$ than the reference baseline. We also see this trend across various face detection models including Facebook's Deepface\footnote{We used an open-source version of Deepface \cite{serengil2021lightface} since the model itself is not publicly available.} \cite{taigman2014deepface} and Google's FaceNet \cite{schroff2015facenet} where the similarity increased by $0.175$ and $0.151$ respectively across all the users and closed-ended tasks. 

% As a secondary analysis similar to the open-ended task, we compare the similarity of the user-generated direction to the target direction with the similarities of $1000$ randomly selected directions. We then report the mean ranking across users. In all of 36 tasks (three tasks per 12 participants), the participant-generated images ranked top-20. In 33 tasks out of 36,
% the participant-generated images ranked top-5. These two analyses show that participants successfully find a similar direction to the one that they are given. 

% \textit{User Behavior}

% For the closed-ended tasks, average number of scatters per task is $1.64$, the average number of times they go back to undo scatter per task is $0.53$. That being said, the standard deviation of number of scatter is $1.53$ across users. Which shows that some users scatter significantly more than the others. The average number of directions tested per task is $6.61$. On average when these directions are being tested, the strength of the direction is changed $3.23$ times. The average time to completion is $7$ minutes and $16$ seconds per task. Participants spent $37.4\%$ of their time on looking at directions either trying to figure out what to scatter or to find a direction of interest. They spent $45.0\%$ of their time testing the directions. The rest of the time, which is $17.6\%$, is spent on highlighting. The average number of changes to the number of clusters is $1.81$. Participants use different number of clusters and are comfortable with 6 to 9 clusters. Participants only asked for more images $0.56$ times per task. 

% All the observations we have for open-ended tasks can also be said for close-ended tasks. One interesting thing to note is almost every participant stated that closed-ended tasks were harder than the open-ended ones since they needed to be more specific. Looking for a more specific direction might explain the increase in number of scatters. That being said the standard deviation of number of scatters is also higher in closed-ended tasks, which shows how some participants did not adjust and did not scatter as much. 


% easy
% , where (s)he somewhat disagreed that the tool was easy to use. P9 said: 'I had too many faces, information to process'. P9 thought that it was hard to know how to improve the directions without getting overwhelmed with information. That being said significant portion of the participants thought the tool was easy to use.  Overall, participants were able to find meaningful directions in an hour long study with a short tutorial at the beginning. Their response also highlights how easy it is to start using \gz.

% success


% tlx

% P1: 'The previous steps help me to find the direction but you still need to figure out the strength. I also utilized the negative weights to confirm the direction.'

% P12: 'You can experiment with the magnitude of the vector. It allowed me to try different combinations and helped me build my intuition about the direction. Especially, going negative direction helped me convince myself. Wish it was continuous.'

% P10: 'Going from negative to the positive was informative. Fine-tuning was also really helpful. If you can find the opposite direction, you could still use it at the test area to find the direction.'

% P8: 'You can directly see the final outcome of your choice. Some images I could decrease the effect to get a better image. When you make it negative, you could truly understand the effect of the direction.'

% P6: 'I could also see the directions on other images. So I have an idea about how well it works generally. I also like you could choose the opposite direction, for example in the last task I could not find the asked direction. Instead I found an opposite direction and used a negative weight on the test area.'

% P5: 'There are 2 validations.
% 1) You can see other images and how direction changes them
% 2) Going negative weight and seeing the transition also helped.
% You could show -5 as well as +5 at the test area.'

% P11: 'I have a chance to change the strength of the directions, which helped me understand what is going on.'

% P4: 'I used this a lot. It helped me understand the directions. Changing the weights from negative to positive helped a lot. Also other images were showing the effect of the direction. It helped me identify entangled features (when I try to make someone happy, their skin tone also changes).'


% This allowed us to select, amongst the 1000 random-direction-generated images, the top-10 images with the highest increase.


    %Further, for each editing goal, we also measured diversity by performing a pairwise comparison amongst all participants' found directions, \eg to show whether participants used \gz to find different ways of making a face happier.
    


% \subsubsection{Open-Ended Tasks} \hfill\\

% \subsubsection{User Performance}

% The cosine similarities of the given text prompts -old, happy and surprised- and the found directions are $0.314 \pm 0.131$, $0.244 \pm  0.189$ and $0.500 \pm 0.072$ respectively according to the CLIP model. To put these numbers into perspective, we sampled $1000$ random directions and analyzed them with the open-source Deepface tool \cite{serengil2021lightface}]. This tool can extract emotions as well as guess the age of the face. Using this tool we identified the best performing $10$ directions for the old, happy and surprised directions. More specifically, we checked the increase in estimated age when these $1000$ directions are applied to the reference image. For happy and surprised, we checked the increase in confidence scores of the respective emotions. Using these values, we were able to identify the best performing directions for each task. Then separately for each task, we test these $10$ pre-selected directions on the CLIP model for cosine similarities with text descriptions as explained in Section~\ref{open_ended_explanation}. Their averages are $0.194 \pm 0.099$, $0.085 \pm 0.106$ and $0.387 \pm 0.172$ respectively, which are all lower than user-generated images. This analysis puts emphasis on how hard is it to search the space of directions. Random sampling and filtering through another AI model is inferior to our user-in-the loop approach by a significant margin.

% % As a secondary analysis, we also looked in to where the participant-generated images rank in previously sampled $1000$ directions. We used the same CLIP metric to keep the consistency across both analyses. In all of $36$ tasks (three tasks per $12$ participants), the participant-generated images ranked top-50. In $30$ tasks out of $36$, the participant-generated images ranked top-10. This result strengthens our observation from the prior analysis.



%(how participants felt successful that their found directions achieved the editing goal)
% \missingfigure{Bar chart for questionnaire can be seen at Figure \xx.}


==> fig_teaser.tex <==
\fg{fig1}{fig1}{1.0}{.}
